Gastric-X: A Multimodal Multi-Phase Benchmark Dataset for Advancing Vision-Language Models in Gastric Cancer Analysis

Recent vision-language models (VLMs) have shown strong generalization and multimodal reasoning abilities in natural domains. However, their application to medical diagnosis remains limited by the lack of comprehensive and structured datasets that capture real clinical workflows. To advance the development of VLMs for clinical applications, particularly in gastric cancer, we introduce Gastric-X, a large-scale multimodal benchmark for gastric cancer analysis providing 1.7K cases. Each case in Gastric-X includes paired resting and dynamic CT scans, endoscopic image, a set of structured biochemical indicators, expert-authored diagnostic notes, and bounding box annotations of tumor regions, reflecting realistic clinical conditions. We systematically examine the capability of recent VLMs on five core tasks: Visual Question Answering (VQA), report generation, cross-modal retrieval, disease classification, and lesion localization. These tasks simulate critical stages of clinical workflow, from visual understanding and reasoning to multimodal decision support. Through this evaluation, we aim not only to assess model performance but also to probe the nature of VLM understanding: Can current VLMs meaningfully correlate biochemical signals with spatial tumor features and textual reports? We envision Gastric-X as a step toward aligning machine intelligence with the cognitive and evidential reasoning processes of physicians, and as a resource to inspire the development of next-generation medical VLMs.

==> rebuttal/clinical.tex <==

\begin{table}[h]
\centering
\small
\vspace{-0.1in}
\setlength{\tabcolsep}{4 pt}
\caption{Clinician evaluation (0--100 scale, mean$\pm$std).}
\label{tab:clinician_manual_eval}
\vspace{-0.1in}
\resizebox{0.25\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
\textbf{Evaluator} 
& \textbf{Semantic Completeness (\%)} 
& \textbf{TNM Utility (\%)} 
\\
\midrule
Clinician 1 
& 76.2 $\pm$ 8.5 
& 78.5 $\pm$ 7.2 
\\

Clinician 2 
& 77.8 $\pm$ 9.1 
& 79.2 $\pm$ 8.3 
\\
Clinician 3 
& 78.1 $\pm$ 8.7 
& 78.9 $\pm$ 7.9 
\\
\bottomrule
\end{tabular}
}
\vspace{-0.15in}
\end{table}

==> rebuttal/encoder.tex <==

\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\vspace{-0.1in}
\caption{Comparing separate vs. shared vision encoders. }
\vspace{-0.1in}
\label{tab:encoder_ablation}
\resizebox{0.3\textwidth}{!}{%
\begin{tabular}{l|cc|cc|c}
\toprule
\multirow{2}{*}{\textbf{Architecture}} 
& \multicolumn{2}{c|}{\textbf{VQA}} 
& \multicolumn{2}{c|}{\textbf{TNM Staging}} 
& \multirow{2}{*}{\textbf{Params}} \\
\cline{2-5}
& Acc (\%) &  F1 (\%) & F1 (\%) & AUC (\%) & \\
\midrule
Separate Encoders 
& 83.7 $\pm$ 2.1 
& 79.2 $\pm$ 2.4 
& 82.1 $\pm$ 2.6 
& 89.8 $\pm$ 1.4 
& 412M \\
% \midrule
Shared Encoder (ours) 
& \textbf{84.6 $\pm$ 1.9} 
& \textbf{79.9 $\pm$ 2.1} 
& \textbf{83.2 $\pm$ 2.3} 
& \textbf{90.8 $\pm$ 1.2} 
& \textbf{223M} \\
\bottomrule
\end{tabular}
}
\vspace{-0.15in}
\end{table}



==> rebuttal/more_result.tex <==


\begin{table}[h]
\centering
\vspace{-0.1in}
\caption{Comparison with SOTA models.}
\label{tab:sota}
\vspace{-0.1in}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{l|cccc|cccc}
\toprule
\multirow{2}{*}{Model} 
& \multicolumn{4}{c|}{Visual Question Answering (VQA)} 
& \multicolumn{4}{c}{TNM Stage Prediction} \\
\cline{2-9}
& Prec. & Acc. & F1 & AUC (\%) 
& Prec. & Rec. & F1 & AUC (\%) \\
\midrule
MedGemma 
& 79.4 $\pm$ 2.8 & 78.1 $\pm$ 2.3 & 78.7 $\pm$ 2.4 & 88.9 $\pm$ 1.3
& 82.6 $\pm$ 3.1 & \textbf{84.1 $\pm$ 2.7} & 83.3 $\pm$ 2.8 & 88.4 $\pm$ 1.6 \\

HuatuoGPT 
& 78.2 $\pm$ 3.0 & 76.8 $\pm$ 2.6 & 77.4 $\pm$ 2.7 & 87.1 $\pm$ 1.5
& 80.9 $\pm$ 3.5 & 82.3 $\pm$ 3.0 & 81.6 $\pm$ 3.1 & 86.9 $\pm$ 1.8 \\

Qwen2.5-VL 
& 77.5 $\pm$ 3.1 & 77.9 $\pm$ 2.7 & 77.6 $\pm$ 2.8 & 85.6 $\pm$ 1.7
& 76.8 $\pm$ 3.8 & 75.4 $\pm$ 3.3 & 76.1 $\pm$ 3.4 & 82.3 $\pm$ 2.1 \\

InternVL3 
& 75.6 $\pm$ 3.4 & 75.1 $\pm$ 3.0 & 75.3 $\pm$ 3.1 & 83.8 $\pm$ 1.9
& 74.2 $\pm$ 4.0 & 73.5 $\pm$ 3.6 & 73.8 $\pm$ 3.7 & 80.6 $\pm$ 2.4 \\

GPT-5 
& \textbf{80.1 $\pm$ 2.6} & \textbf{80.8 $\pm$ 2.1} & 79.9 $\pm$ 2.3 & 86.4 $\pm$ 1.8
& 75.3 $\pm$ 4.1 & 71.8 $\pm$ 3.9 & 73.5 $\pm$ 3.8 & 79.2 $\pm$ 2.6 \\

Gemini-2.5-Pro 
& 79.6 $\pm$ 2.7 & 80.2 $\pm$ 2.2 & 79.4 $\pm$ 2.4 & 86.9 $\pm$ 1.7
& 76.1 $\pm$ 4.0 & 72.9 $\pm$ 3.7 & 74.4 $\pm$ 3.6 & 80.1 $\pm$ 2.5 \\

\midrule
\textbf{X2-VLM-Med (ours)} 
& 77.8 $\pm$ 2.5 & 84.6 $\pm$ 1.9 & \textbf{79.9 $\pm$ 2.1} & \textbf{91.5 $\pm$ 1.1}
& \textbf{83.9 $\pm$ 2.4} & 82.6 $\pm$ 2.6 & \textbf{83.2 $\pm$ 2.3} & \textbf{90.8 $\pm$ 1.2} \\

% \midrule
% GPT Healthcare (planned) 
% & -- & -- & -- & --
% & -- & -- & -- & -- \\

% MedGemini (planned) 
% & -- & -- & -- & --
% & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
}
\vspace{-0.1in}
\end{table}

==> rebuttal/vqa_finegrain.tex <==

\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\vspace{-0.1in}
\caption{Performance on fine-grained VQA sub-tasks.}
\vspace{-0.1in}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l c c c c c}
\hline
\textbf{VQA Question Type} & \textbf{Metric} & \textbf{LLaVA-Med} & \textbf{MedVInT} & \textbf{Med-Flamingo} & \textbf{X2-VLM-Med} \\
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}
Visual Attribute Recognition \\
{\footnotesize (location, size trend, enhancement)}
\end{tabular}}
& Acc $\uparrow$ & 74.8 & 76.3 & 78.5 & \textbf{82.6} \\
& F1 $\uparrow$  & 71.9 & 73.8 & 76.2 & \textbf{80.4} \\
& AUC $\uparrow$ & 86.1 & 87.4 & 88.9 & \textbf{91.8} \\
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}
Clinical Fact Verification \\
{\footnotesize (presence / absence, yes--no)}
\end{tabular}}
& Acc $\uparrow$ & 78.6 & 80.1 & 82.4 & \textbf{86.3} \\
& F1 $\uparrow$  & 76.5 & 78.0 & 80.7 & \textbf{84.1} \\
& AUC $\uparrow$ & 88.3 & 89.6 & 91.2 & \textbf{93.4} \\
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}
Cross-modal Reasoning \\
{\footnotesize (image + lab + report)}
\end{tabular}}
& Acc $\uparrow$ & 72.4 & 74.6 & 76.9 & \textbf{81.2} \\
& F1 $\uparrow$  & 69.8 & 72.0 & 74.5 & \textbf{79.0} \\
& AUC $\uparrow$ & 84.9 & 86.7 & 88.3 & \textbf{91.1} \\
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}
Numerical / Staging-related \\
{\footnotesize (T/N/M cues, ordinal reasoning)}
\end{tabular}}
& Acc $\uparrow$ & 68.9 & 71.2 & 73.4 & \textbf{77.5} \\
& F1 $\uparrow$  & 65.7 & 68.3 & 70.6 & \textbf{75.1} \\
& AUC $\uparrow$ & 82.6 & 84.1 & 85.8 & \textbf{89.2} \\
\hline
\end{tabular}
}
\vspace{-0.15in}
\label{tab:vqa_finegrained}
\end{table}



==> table/supp_tables_plain.tex <==
% Auto-generated plain table version
\begin{table*}[t]
\centering
\begin{tabular}{l p{6cm} l p{6cm}}
\toprule
Item & Description & Item & Description \\
\midrule
Hospital ID (De-identified) & Anonymized hospitalization identifier & Patient Name (De-identified) & Anonymized patient name code \\
Sex & Biological sex & Age (De-identified) & Age at admission (de-identified) \\
Bed Number (De-identified) & Anonymized bed assignment & Surgery Date (De-identified) & Date of surgery (de-identified) \\
Imaging ID & CT imaging identifier & CT Description & Radiology morphological description \\
CBC: Test Date & Date of CBC test & CBC: White Blood Cell Count & White blood cell count (×10^9/L) \\
CBC: Neutrophil Count & Absolute neutrophil count (×10^9/L) & CBC: Neutrophil Ratio & Neutrophil percentage (\%) \\
CBC: Lymphocyte Count & Absolute lymphocyte count (×10^9/L) & CBC: Lymphocyte Ratio & Lymphocyte percentage (\%) \\
CBC: Hemoglobin & Hemoglobin concentration (g/L) & CBC: Platelet Count & Platelet count (×10^9/L) \\
Biochemistry: Test Date & Date of biochemistry test & Biochemistry: Fasting Glucose & Fasting plasma glucose (mmol/L) \\
Biochemistry: Prealbumin & Serum prealbumin (mg/L) & Biochemistry: ALT & Alanine aminotransferase (U/L) \\
Biochemistry: AST & Aspartate aminotransferase (U/L) & Biochemistry: Total Protein & Total serum protein (g/L) \\
Biochemistry: Albumin & Serum albumin (g/L) & Biochemistry: Total Bilirubin & Total bilirubin (µmol/L) \\
Biochemistry: Direct Bilirubin & Direct bilirubin (µmol/L) & Biochemistry: Creatinine & Serum creatinine (µmol/L) \\
Biochemistry: Urea (BUN) & Blood urea nitrogen (mmol/L) & Tumor Markers: Test Date & Date of tumor marker test \\
Tumor Markers: AFP & Alpha-fetoprotein (AFP) & Tumor Markers: CEA & Carcinoembryonic antigen (CEA) \\
Tumor Markers: CA125 & Cancer antigen 125 (CA125) & Tumor Markers: CA724 & Cancer antigen 724 (CA724) \\
Tumor Markers: CA199 & Cancer antigen 19-9 (CA19-9) & Past Medical History: Conditions (Not Used) & Past medical conditions (record retained but not used in experiments) \\
Surgical/Trauma History (Not Used) & Prior surgical or trauma history (retained but not used) & Hospital ID (De-identified) & Anonymized hospitalization identifier \\
Patient Name (De-identified) & Anonymized patient name code & Sex & Biological sex \\
年龄 & Clinical variable & 床号 & Clinical variable \\
手术日期 & Clinical variable & Resection Range & Extent of resection \\
Gastrointestinal Reconstruction & Type of reconstruction after resection & Occupation & Patient occupation (anonymized) \\
Education Level & Highest educational attainment & Marital Status & Marital status \\
Ethnicity & Ethnic group & Admission Method & Mode of hospital admission \\
Insurance Status & Medical insurance coverage & ID Number (De-identified) & Identification document number (anonymized) \\
Contact Number (De-identified) & Contact phone (anonymized) & Surgery Admission Date (De-identified) & Date of admission for surgery (de-identified) \\
Surgery Discharge Date (De-identified) & Date of discharge after surgery (de-identified) & Surgery Hospitalization Cost & Total cost for surgical hospitalization (local currency) \\
Admission Temperature & Body temperature at admission (°C) & Admission Pulse & Pulse rate at admission (beats/min) \\
Admission Respiration & Respiratory rate at admission (breaths/min) & Admission Systolic Pressure & Systolic blood pressure at admission (mmHg) \\
Admission Diastolic Pressure & Diastolic blood pressure at admission (mmHg) & Height & Height (cm) \\
Weight & Weight (kg) & BMI & Body mass index (kg/m^2) \\
General Condition & Clinical performance status (qualitative) & Weight Loss & Recent unintended weight loss \\
Reduced Food Intake & Decrease in oral intake & Smoking Status & Current/former/never smoker \\
Drinking Status & Alcohol consumption status & Endoscopy Date (De-identified) & Date of gastroscopy (de-identified) \\
Endoscopy Tumor Location & Tumor location observed in endoscopy & Endoscopy Tumor Size & Tumor size measured in endoscopy (cm) \\
Endoscopy Gross Type & Endoscopic macroscopic classification & Endoscopy Biopsy Pathology & Biopsy-based pathological diagnosis \\
Endoscopy Appearance & Endoscopic visual findings & Chief Surgeon (De-identified) & Primary operating surgeon (anonymized) \\
First Assistant (De-identified) & Primary assistant surgeon (anonymized) & Surgery Nature & Elective/emergency \\
Surgery Mode & Open or minimally invasive & Lymphadenectomy Extent & Extent of lymph node dissection \\
Combined Resections & Concurrent organ resections & Surgery Start Time (De-identified) & Operation start time (de-identified) \\
Surgery End Time (De-identified) & Operation end time (de-identified) & Surgery Duration & Total operative time (minutes) \\
Intraoperative Blood Loss & Estimated blood loss (mL) & Transfused Red Blood Cells & Units of RBC transfused \\
Transfused Plasma & Volume of plasma transfused & Intraoperative Transfusion & Any transfusion during surgery \\
Residual Tumor (Intraoperative) & Macroscopic residual tumor status & Drainage Tube & Presence of drainage tube \\
Additional Procedures & Other intraoperative procedures & Tumor Anatomical Location & Anatomical site of the tumor \\
Tumor Lateral Position & Lateral orientation of tumor & Maximum Tumor Diameter & Maximal tumor diameter (cm) \\
Serosal Invasion & Serosal layer involvement (Y/N) & Gross Tumor Type & Macroscopic tumor classification \\
Linitis Plastica & Presence of linitis plastica (Y/N) & Perigastric Lymph Nodes & Status of perigastric nodes \\
Liver Metastasis & Presence of hepatic metastases (Y/N) & Adjacent Organ Invasion & Invasion of neighboring organs (Y/N) \\
Peritoneal Seeding & Peritoneal metastasis (Y/N) & Ascites & Presence of ascites (Y/N) \\
Pathology ID (De-identified) & Anonymized pathology specimen identifier & Tumor Size - Long Axis & Pathology long-axis measurement (cm) \\
Tumor Size - Short Axis & Pathology short-axis measurement (cm) & Tumor Size - Height & Tumor height (cm) \\
Primary Histologic Type & Main histological subtype & Histologic Grade & Tumor differentiation grade \\
Additional Histologic Type & Other histologic components & Distance to Proximal Margin & Distance from tumor to proximal margin (cm) \\
Distance to Distal Margin & Distance from tumor to distal margin (cm) & Specimen Proximal Margin & Proximal margin status (specimen) \\
Specimen Distal Margin & Distal margin status (specimen) & Perineural Invasion & Perineural invasion (Y/N) \\
Vascular Cancer Thrombus & Vascular invasion / intravascular tumor thrombus (Y/N) & Greater Omentum Invasion & Invasion of greater omentum (Y/N) \\
Lesser Omentum Invasion & Invasion of lesser omentum (Y/N) & Greater Omentum Metastasis & Metastasis to greater omentum (Y/N) \\
Lesser Omentum Metastasis & Metastasis to lesser omentum (Y/N) & Multifocal Tumors & Presence of multiple tumor foci (Y/N) \\
Positive Lymph Nodes & Number of positive lymph nodes & Dissected Lymph Nodes & Total number of dissected lymph nodes \\
T Stage & Pathological T category & N Stage & Pathological N category \\
M Stage & Pathological M category & Overall Stage & Overall pathologic stage \\
Surgical Radicality & R0/R1/R2 resection status & Group 1 Positive & Group 1 positive node count \\
Group 1 Dissected & Group 1 dissected count & Group 2 Positive & Group 2 positive node count \\
Group 2 Dissected & Group 2 dissected count & Group 3 Positive & Group 3 positive node count \\
Group 3 Dissected & Group 3 dissected count & Group 4 Positive & Group 4 positive node count \\
Group 4 Dissected & Group 4 dissected count & Group 5 Positive & Group 5 positive node count \\
Group 5 Dissected & Group 5 dissected count & Group 6 Positive & Group 6 positive node count \\
Group 6 Dissected & Group 6 dissected count & Groups 7/8/9 Positive & Groups 7/8/9 positive node count \\
Groups 7/8/9 Dissected & Groups 7/8/9 dissected count & Greater Curvature Positive & Positive nodes on greater curvature \\
Greater Curvature Dissected & Dissected nodes on greater curvature & Lesser Curvature Positive & Positive nodes on lesser curvature \\
Lesser Curvature Dissected & Dissected nodes on lesser curvature & Other Stations Positive & Other nodal station positive count \\
Other Stations Dissected & Other nodal station dissected count & Ki-67 & Proliferation index (IHC) \\
HER2 Status & HER2 receptor status (IHC) & CLDN Status & Claudin expression status \\
MLH1 & MLH1 expression (IHC) & PMS2 & PMS2 expression (IHC) \\
MSH2 & MSH2 expression (IHC) & MSH6 & MSH6 expression (IHC) \\
EBER & EBV-encoded RNA by ISH & PD-L1 Score & PD-L1 immunohistochemistry score \\
MMR Status & Mismatch repair status & PD-L1 Status & PD-L1 categorical status \\
Complication Severity & Clavien–Dindo grade & Secondary Surgery & Reoperation required (Y/N) \\
Complication Occurrence & Any postoperative complication (Y/N) & Complication Present & Whether complication occurred (Y/N) \\
Severe Complication Occurrence & Severe complication (Y/N) & Total Hospital Stay (Days) & Total days hospitalized for surgery \\
Postoperative Stay (Days) & Days hospitalized after surgery & Preoperative Transfusion & Any transfusion before surgery \\
Postoperative Transfusion & Any transfusion after surgery & Postoperative Fever & Fever after surgery (Y/N) \\
Fever Days & Number of days with postoperative fever & Complication Category & Type/category of complication \\
Intervention & Management or treatment measures & Complication Notes & Additional notes on complications \\
\bottomrule
\end{tabular}
\end{table*}

